Microlocal Theory of Legendrian Links and Cluster Algebras

We show the existence of quasi-cluster $\mathcal{A}$-structures and cluster Poisson structures on moduli stacks of sheaves with singular support in the alternating strand diagram of grid plabic graphs by studying the microlocal parallel transport of sheaf quantizations of Lagrangian fillings of Legendrian links. The construction is in terms of contact and symplectic topology, showing that there exists an initial seed associated to a canonical relative Lagrangian skeleton. In particular, mutable cluster $\mathcal{A}$-variables are intrinsically characterized via the symplectic topology of Lagrangian fillings in terms of dually $\mathbb{L}$-compressible cycles. New ingredients are introduced throughout this work, including the initial weave associated to a grid plabic graph, cluster mutation along a non-square face of a plabic graph, the concept of the sugar-free hull, and the notion of microlocal merodromy. Finally, a contact geometric realization of the DT-transformation is constructed for shuffle graphs, proving cluster duality for the cluster ensembles.

==> 5_gallery_of_examples.tex <==
\section{Gallery of Examples}\label{sec:}

%\color{blue} TO DO: Include many cool examples. In particular, we should include that family given by ``bending'', which gives twist knots if I recall correctly and the mutable part of the cluster algebra remains the same. In any case, we have tons of good examples, so surely we can choose a few (maybe about five) which illustrate what we are doing and make it apparent that this weave-and-cluster relation is fruitful.\color{black}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%\begin{example}\label{ex:m52_Continued}{\bf Continue Example \ref{ex:m52_ClusterCoord} here: explain the irreducibility and the sugar free hull, which are easy from there, and the do one mutation. See Figure \ref{fig:Example_m52_ClusterCoord2}}
%\end{example}
\subsection{Primer: an $m(5_2)$ Example}\label{ssec:m(5_2)} Let us consider the following shuffle graph $\bG$ once more. The associated GP-link $\Lambda=\Lambda(\bG)$ is a Legendrian link of smooth knot type $m(5_2)$ (see also Figures \ref{fig:Example_m52} and \ref{fig:Example_Twist} (upper-left)). The weave $\ww=\ww(\bG)$ drawn in Figure \ref{fig:Example_m52} simplifies by undoing a candy twist to the weave on the right below.
\begin{figure}[H]
    \centering
    \begin{tikzpicture}[scale=1.5]
    \horline[](0,3.5,0);
    \horline[](0,3.5,1.5);
    \vertbar[](0.5,0,1.5);
    \vertbar[](3,0,1.5);
    \horline[](1,2.5,0.75);
    \vertbar[](1.5,0,0.75);
    \vertbar[](2,0.75,1.5);
    \node at (0.75,1.25) [] {$f_1$};
    \node at (2.75,0.25) [] {$f_2$};
    \end{tikzpicture}\quad \quad \quad \quad 
    \begin{tikzpicture}[scale=1.5]
    \draw [blue] (0,0.75) -- (0.5,0.75) -- (0.5,1.5);
    \draw [red] (1,0) -- (1,0.5) -- (1.5,0.5) -- (1.75,0.75) -- (1.5,1) -- (1.5,1.5);
    \draw [red] (1.5,1) -- (1,1) -- (1,1.5);
    \draw [blue] (2.5,0) -- (2.5,0.5) -- (2,0.5) -- (1.75,0.75) -- (2,1) -- (2,1.5);
    \draw [blue] (2,1) -- (2.5,1) -- (2.5,1.5);
    \draw [red] (3,1.5) -- (3,0.75) -- (3.5,0.75);
    \draw [blue] (0.5,0.75) -- (1.75,0.75);
    \draw [red] (1.75,0.75) -- (3,0.75);
    \draw [dotted, thick] (0.5,0.75) -- node [left] {\footnotesize{$1$}} (0,1.5);
    \draw [dotted,thick] (1.5,1) -- (1.3,1.2) node [below] {\footnotesize{$3$}} -- (0.3,1.2) -- (0,1.5);
    \draw [dotted,thick] (2,1) -- (1.8,1.3) node [below] {\footnotesize{$2$}} -- (0.35,1.3) -- (0,1.5);
    \draw [dotted,thick] (3,0.75) --(2.8,0.9) node [left] {\footnotesize{$2$}} -- (2.8,1.4) -- (0.4,1.4) -- (0,1.5);
    \node at (0,1.5) [] {$\ast$};
    \end{tikzpicture}
    \caption{$m(5_2)$ as a GP-link and its initial weave together with a compatible set of sign curves.}
    \label{fig:m(5_2) with sign curves}
\end{figure}

Let us name the naive absolute cycles as $\gamma_i:=\partial f_i$ for $i=1,2$. There is only one sugar-free hull $f_1\cup f_2$. Thus, the set of initial absolute cycles consists of only one element, namely $\delta:=\gamma_1+\gamma_2$; it embeds in the initial weave as the unique long $\sf I$-cycle between the left most and the right most trivalent weave vertices.

Since $m(5_2)$ is a knot, we only need to put one marked point on its boundary. Let us put it on the lowest strand at upper left hand corner. Among the four Type 2 columns, only the right most one is critical. Let us fix a compatible set of sign curves as depicted in the right picture in Figuer \ref{fig:m(5_2) with sign curves}.


Since the unique marked point is the end point of four distinct sign curves, there is no need to change the decorations across this marked point. By reading the boundary weave lines, we see that $\cM(\Lambda(\bG))$ is the configuration of $10$ flags satisfying the relative position conditions described in Example \ref{exmp:m(5_2) flag configurations}. 

The framing data decorate each flag by associating a non-zero form to each subspace. Following the cyclic order in Example \ref{exmp:m(5_2) flag configurations}, we name them as follows. The left most decorated flag is associated with the sector in which the unique marked point is located. Note that the sign changes on the decorations are in accordance with Equation \eqref{eq:signs_of_decorations}.
\[
\begin{tikzpicture}
\node (0) at (0,0) [] {$\begin{pmatrix}\det \\ \alpha_0 \\ v_0\end{pmatrix}$};
\node (1) at (2,1) [] {$\begin{pmatrix}-\det \\ -\alpha_0 \\ v_1\end{pmatrix}$};
\node (2) at (4,1) [] {$\begin{pmatrix} \det \\ \alpha_1 \\ v_1\end{pmatrix}$};
\node (3) at (6,1) [] {$\begin{pmatrix} -\det \\ \alpha_2 \\ v_1\end{pmatrix}$};
\node (4) at (8,1) [] {$\begin{pmatrix} \det \\ -\alpha_2 \\ v_2\end{pmatrix}$};
\node (5) at (10,1) [] {$\begin{pmatrix} -\det \\ \alpha_2 \\ v_3\end{pmatrix}$};
\node (6) at (12,1) [] {$\begin{pmatrix} \det \\ \alpha_3 \\ v_3\end{pmatrix}$};
\node (7) at (14,0) [] {$\begin{pmatrix} -\det \\ \alpha_4 \\ v_3\end{pmatrix}$};
\node (8) at (10,-1) [] {$\begin{pmatrix} \det \\ -\alpha_4 \\ v_4\end{pmatrix}$};
\node (9) at (4,-1) [] {$\begin{pmatrix} -\det \\ -\alpha_0 \\ v_4\end{pmatrix}$};
\draw (0) -- node[above left,blue] {$s_1$} (1);
\draw (1) -- node[above,red] {$s_2$} (2);
\draw (2) -- node[above,red] {$s_2$} (3);
\draw (3) -- node[above,blue] {$s_1$} (4);
\draw (4) -- node[above,blue] {$s_1$} (5);
\draw (5) -- node[above,red] {$s_2$} (6);
\draw (6) -- node[above right,red] {$s_2$} (7);
\draw (7) -- node[below,blue] {$s_1$} (8);
\draw (8) -- node[below,red] {$s_2$} (9);
\draw (9) -- node[below left,blue] {$s_1$} (0);
\end{tikzpicture}
\]
In addition, by Lemma \ref{lem: local crossing value}, we have the following identities
\[
\alpha_0=v_4\wedge v_0=v_1\wedge v_0, \quad \quad \alpha_2=v_2\wedge v_1=v_2\wedge v_3, \quad \quad \alpha_4=v_4\wedge v_3,
\]
\[
\det=(-\alpha_0)\overset{v_1}{\wedge}\alpha_1=\alpha_2\overset{v_1}{\wedge}\alpha_1=\alpha_2\overset{v_3}{\wedge} \alpha_3=\alpha_4\overset{v_3}{\wedge}\alpha_3=(-\alpha_0)\overset{v_4}{\wedge}(-\alpha_4).
\]
Suppose $\alpha_1=u\wedge v_1$ and $\alpha_3=w\wedge v_3$. Then from the $\det$ identity above, we see that
\[
\det=v_0\wedge u\wedge v_1=v_2\wedge u\wedge v_1=v_2\wedge w\wedge v_3=v_4\wedge w\wedge v_3=v_0\wedge v_3\wedge v_4.
\]
%\[
%\det=v_0\wedge u\wedge v_4=v_2\wedge u\wedge v_3=v_2\wedge w\wedge v_1=v_0\wedge v_3\wedge v_1.
%\]

Next let us define the naive microlocal merodromies. We have a few possible choices for the dual naive relative cycle for each of the two faces. In Figure \ref{fig: choices for naive relative cycles}, we draw a few possible choices for the face $f_2$ in purple.
\begin{figure}[H]
\begin{tikzpicture}[scale=2.5]
    \draw [blue] (0,0.75) -- (0.5,0.75) -- (0.5,1.5);
    \draw [red] (1,0) -- (1,0.5) -- (1.5,0.5) -- (1.75,0.75) -- (1.5,1) -- (1.5,1.5);
    \draw [red] (1.5,1) -- (1,1) -- (1,1.5);
    \draw [blue] (2.5,0) -- (2.5,0.5) -- (2,0.5) -- (1.75,0.75) -- (2,1) -- (2,1.5);
    \draw [blue] (2,1) -- (2.5,1) -- (2.5,1.5);
    \draw [red] (3,1.5) -- (3,0.75) -- (3.5,0.75);
    \draw [blue] (0.5,0.75) -- (1.75,0.75);
    \draw [red] (1.75,0.75) -- (3,0.75);
    \draw [dotted, thick] (0.5,0.75) -- (0,1.5);
    \draw [dotted,thick] (1.5,1) -- (1.3,1.2) -- (0.3,1.2) -- (0,1.5);
    \draw [dotted,thick] (2,1) -- (1.8,1.3)-- (0.35,1.3) -- (0,1.5);
    \draw [dotted,thick] (3,0.75) --(2.8,0.9)  -- (2.8,1.4) -- (0.4,1.4) -- (0,1.5);
    \draw [purple, dashed,thick] (2.75,-0.25) -- node [below right] {\footnotesize{$1$}} (2.75,1.75);
    \draw [purple, dashed,thick] (2.3,-0.25) -- (2.3,1.75);
    \node [purple] at (2.3,0.5) [above right] {\footnotesize{$0$}};
    \node [purple]at (2.3,0.75) [above right] {\footnotesize{$1$}};
    \node[purple] at (2.3,1) [above right] {\footnotesize{$1$}};
    \draw [purple, dashed,thick] (2.2,-0.25) -- (2.2,1.75);
    \node [purple] at (2.2,0.5) [above left] {\footnotesize{$1$}};
    \node [purple]at (2.2,0.75) [above left] {\footnotesize{$1$}};
    \node[purple] at (2.2,1) [above left] {\footnotesize{$0$}};
    \draw [purple, dashed,thick] (1.85,-0.25) -- (1.85,1.75);
    \node [purple] at (1.85,0.5) [above right] {\footnotesize{$1$}};
    \node [purple]at (1.85,0.75) [above right] {\footnotesize{$1$}};
    \node[purple] at (1.85,1) [above right] {\footnotesize{$0$}};
    \draw [teal, dashed,thick] (0.75,-0.25) -- node [above left] {\footnotesize{$1$}} (0.75,1.75);
    \node at (0,1.5) [] {$\ast$};
    \node at (0.25,1.5) [] {\footnotesize{$1$}};
    \node at (0.85,1.5) [] {\footnotesize{$2$}};
    \node at (1.25,1.5) [] {\footnotesize{$3$}};
    \node at (1.75,1.5) [] {\footnotesize{$2$}};
    \node at (2.25,1.5) [] {\footnotesize{$1$}};
    \node at (2.65,1.5) [] {\footnotesize{$2$}};
    \end{tikzpicture}
    \caption{Possible choices for naive relative cycles.}\label{fig: choices for naive relative cycles}
    \end{figure}
We can now apply Proposition \ref{prop: A_f are regular functions} to write down expressions for these microlocal merodromies. We have label the sheet index for the sign curves to help us keep track of whether these relative 1-cycles cross the sign curves or not. The resulting expressions are the following, and it is not hard to verify that they are all equal.
\[
A_2=\frac{v_4\wedge \alpha_2}{-\det}=\frac{v_4\wedge (-\alpha_2)}{\det}=-\frac{v_2\wedge(-\alpha_4)}{\det}=\frac{\alpha_4\overset{v_3}{\wedge}\alpha_2}{-\det}
\]
Similarly, by using the relative 1-cycle in green, one can find that
\[
A_1=-\frac{v_4\wedge v_1}{-\alpha_0}=\frac{v_4\wedge v_1}{\alpha_0}.
\]


Since $\fS(\bG)=\{\delta\}$ is a singleton set but $H_1(L,T)\cong H_1(L)\cong \mathbb{Z}^2$ (Example 3 in Subsection \ref{ssec:AFewExamples}), we need to choose a completion of $\fS(\bG)$ to a basis of $H_1(L)$. One such choice is by adding $\gamma_1$, which gives the following initial quiver (the vertex $\gamma_1$ is frozen).
\[
\begin{tikzpicture}
\node (0) at (0,0) [] {$\delta$};
\node [blue] (1) at (1.5,0) [] {$\gamma_1$};
\draw [->] (1) -- (0);
\end{tikzpicture}
\]
The dual basis to $\{\delta,\gamma_1\}$ is $\{\eta_2,\eta_1-\eta_2\}$. Therefore the initial cluster is
\[
\begin{tikzpicture}
\node (0) at (0,0) [] {$A_2$};
\node [blue] (1) at (1.5,0) [] {$\dfrac{A_1}{A_2}$};
\draw [->] (1) -- (0);
\end{tikzpicture}
\]
In particular, Proposition \ref{prop:A_f/A_g is a unit} implies that 
\[
\frac{A_1}{A_2}=\frac{v_4\wedge v_1}{\alpha_0}\frac{\det}{v_4\wedge v_1\wedge v_2}=\frac{\det}{\alpha_0\wedge v_2}
\]
is a unit. In other words, $\alpha_0\wedge v_2\neq 0$ up to codimension 2 and hence when computing functions on $\FM(\Lambda(\bG),T)$, we may assume that the line $\Span(v_2)$ and the plane $\Span(\alpha_0)$ are always transverse to each other.


Let us compute the cluster $\mathcal{A}$-mutation at $A_2$. According to the cluster $\mathcal{A}$-mutation formula, we should get
\begin{align*}
    A'_2=&\frac{1+\frac{A_1}{A_2}}{A_2}=\frac{\det+\frac{\det}{\alpha_0\wedge v_2}\det}{v_4\wedge v_3\wedge v_2}=\frac{(v_1\wedge v_0\wedge v_2)\det +\det^2}{(v_4\wedge v_3\wedge v_2)(\alpha_0\wedge v_2)}\\
    =&\frac{(v_3\wedge v_0\wedge v_2)(v_4\wedge w\wedge v_3)+(v_2\wedge w\wedge v_3)(v_0\wedge v_3\wedge v_4)}{(v_4\wedge v_3\wedge v_2)(\alpha_0\wedge v_2)}\\
    =&\frac{(v_4\wedge v_2\wedge v_3)(v_0\wedge w\wedge v_3)}{(v_4\wedge v_3\wedge v_2)(\alpha_0\wedge v_2)}\\
    =&\frac{v_0\wedge v_3\wedge w}{\alpha_0\wedge v_2}.
\end{align*}
Note that in the second to the last equality, we used a Pl\"{u}cker relation among the vectors $v_4,v_0,v_2,w$ in $\mathbb{C}^3/\Span(v_3)$. Also, since $\alpha_0\wedge v_2$ never vanishes, we can deduce that $A'_2$ is a regular function on $\FM(\Lambda(\bG),T)$.

Let us also demonstrate how we can compute $A'_2$ via a weave mutation. We first do a weave equivalence to the initial weave to obtain the following weave on the top left, in which the unique long $\sf I$-cycle $\delta$ becomes a short $\sf I$-cycle. We draw a representative of the dual initial relative cycle $\eta_2$ in purple.
\begin{figure}[H]
    \centering
\begin{tikzpicture}[scale=1.5]
    \draw [blue] (0.5,0.75) -- (0.5,1.5);
    \draw [red] (1.75,0.75) -- (1.5,1) -- (1.5,1.5);
    \draw [red] (1.5,1) -- (1,1) -- (1,1.5);
    \draw [blue] (1.75,0.75) -- (2,1) -- (2,1.5);
    \draw [blue] (2,1) -- (2.5,1) -- (2.5,1.5);
    \draw [red] (3,1.5) -- (3,0.5) -- (3.5,0.5);
    \draw [blue] (0.5,0.75) -- (1.75,0.75);
    \draw [red] (1.75,0.75) -- (2.25,0.75) -- (2.5,0.5) -- (2.25,0.25) -- (1.75,0.25) -- (1.5,0) -- (1,0) -- (1,-0.5);
    \draw [red] (2.5,0.5) -- (3,0.5);
    \draw [blue] (0,0.25) -- (1.75,0.25) -- (2,0) -- (2.5,0) -- (2.5,-0.5);
    \draw [red] (1.75,0.75) -- (1.5,0.5) -- (1.75,0.25);
    \draw [blue] (1.75,0.75) -- (2,0.5) -- (1.75,0.25);
    \draw [dotted, thick] (2.5,0.5) -- (0.5,0.5) -- node [left] {\footnotesize{$1$}} (0,1.5);
    \draw [dotted,thick] (1.5,1) -- (1.3,1.2) node [below] {\footnotesize{$3$}} -- (0.3,1.2) -- (0,1.5);
    \draw [dotted,thick] (2,1) -- (1.8,1.3) node [below] {\footnotesize{$2$}} -- (0.35,1.3) -- (0,1.5);
    \draw [dotted,thick] (3,0.5) --(2.8,0.7)  -- (2.8,1.4) node [above right] {\footnotesize{$2$}} -- (0.4,1.4) -- (0,1.5);
    \node at (0,1.5) [] {$\ast$};
    \draw [purple, dashed] (2.75,-0.75) -- node [below left] {\footnotesize{$1$}} (2.75,1.75);
    \end{tikzpicture} \quad \quad\quad \quad
    \begin{tikzpicture}[scale=1.5]
    \draw [blue] (0.5,0.75) -- (0.5,1.5);
    \draw [red] (1.75,0.75) -- (1.5,1) -- (1.5,1.5);
    \draw [red] (1.5,1) -- (1,1) -- (1,1.5);
    \draw [blue] (1.75,0.75) -- (2,1) -- (2,1.5);
    \draw [blue] (2,1) -- (2.5,1) -- (2.5,1.5);
    \draw [blue] (0.5,0.75) -- (1.75,0.75);
    \draw [red] (1.75,0.75) -- (3,0.75) -- (3,1.5);
    \draw [red] (3.5,0.25) --  (1.75,0.25) -- (1.5,0) -- (1,0) -- (1,-0.5);
    \draw [red] (2.75,0.75) -- (2.75,0.25);
    \draw [blue] (0,0.25) -- (1.75,0.25) -- (2,0) -- (2.5,0) -- (2.5,-0.5);
    \draw [red] (1.75,0.75) -- (1.5,0.5) -- (1.75,0.25);
    \draw [blue] (1.75,0.75) -- (2,0.5) -- (1.75,0.25);
    \draw [dotted, thick] (2.75,0.25) -- (2.6,0.35) -- (0.5,0.35) -- node [left] {\footnotesize{$1$}} (0,1.5);
    \draw [dotted,thick] (1.5,1) -- (1.3,1.2) node [below] {\footnotesize{$3$}} -- (0.3,1.2) -- (0,1.5);
    \draw [dotted,thick] (2,1) -- (1.8,1.3) node [below] {\footnotesize{$2$}} -- (0.35,1.3) -- (0,1.5);
    \draw [dotted,thick] (2.75,0.75) --(2.75,1.4) node [above right] {\footnotesize{$2$}} -- (0.4,1.4) -- (0,1.5);
    \node at (0,1.5) [] {$\ast$};
    \draw [purple, dashed] (2.85,1.75) -- (2.85,0.5) -- (2.65,0.5) -- (2.65,-0.75);
    \node [purple] at (2.85,0.75) [below right] {\footnotesize{$-1$}};
    \node [purple] at (2.75,0.5) [below right] {\footnotesize{$1$}};
    \node [purple]at (2.65,0.25) [below left] {\footnotesize{$-1$}};
    \end{tikzpicture}\\
    \begin{tikzpicture}[scale=1.5]
    \draw [blue] (0.5,0.75) -- (0.5,1.5);
    \draw [red] (1.75,0.75) -- (1.5,1) -- (1.5,1.5);
    \draw [red] (1.5,1) -- (1,1) -- (1,1.5);
    \draw [blue] (1.75,0.75) -- (2,1) -- (2,1.5);
    \draw [blue] (2,1) -- (2.5,1) -- (2.5,1.5);
    \draw [blue] (0.5,0.75) -- (1.75,0.75);
    \draw [red] (1.75,0.75) -- (3,0.75) -- (3,1.5);
    \draw [red] (3.5,0.25) --  (1.75,0.25) -- (1.5,0) -- (1,0) -- (1,-0.5);
    \draw [red] (2.75,0.75) -- (2.75,0.25);
    \draw [blue] (0,0.25) -- (1.75,0.25) -- (2,0) -- (2.5,0) -- (2.5,-0.5);
    \draw [red] (1.75,0.75) -- (1.5,0.5) -- (1.75,0.25);
    \draw [blue] (1.75,0.75) -- (2,0.5) -- (1.75,0.25);
    \draw [dotted, thick] (2.75,0.25) -- (2.6,0.35) -- (0.5,0.35) -- node [left] {\footnotesize{$1$}} (0,1.5);
    \draw [dotted,thick] (1.5,1) -- (1.3,1.2) node [below] {\footnotesize{$3$}} -- (0.3,1.2) -- (0,1.5);
    \draw [dotted,thick] (2,1) -- (1.8,1.3) node [below] {\footnotesize{$2$}} -- (0.35,1.3) -- (0,1.5);
    \draw [dotted,thick] (2.75,0.75) --(2.75,1.4) node [above right] {\footnotesize{$2$}} -- (0.4,1.4) -- (0,1.5);
    \node at (0,1.5) [] {$\ast$};
    \draw [purple, dashed] (-0.25,0.5) -- (3.75,0.5);
    \node [purple] at (1.5,0.5) [above left] {\footnotesize{$-1$}};
    \node [purple] at (2.75,0.5) [above right] {\footnotesize{$1$}};
    \node [purple]at (2,0.5) [above right] {\footnotesize{$0$}};
    \end{tikzpicture}
\caption{Mutating the initial weave for $m(5_2)$.}
    \label{fig:mutating initial weave for m(5_2)}
\end{figure}
According to Figure \ref{fig:mutation of relative cycles}, the weave mutation at the short $\sf I$-cycle $\delta$ now produces the weave above on the top right above, together with a new relative cycle $\eta'$ as drawn. But we can homotope $\eta'$ to the purple relative cycle representative in the picture in the second row. By applying Proposition \ref{prop: A_f are regular functions} to the relative cycle representative in the last picture, we see that
\[
A_{\eta'}=-\left.\frac{v_0\wedge \alpha_3}{\det}\right/\frac{v_3\wedge \alpha_0}{\det}=-\frac{v_0\wedge w\wedge v_3}{v_3\wedge v_4\wedge v_0}=\frac{v_0\wedge v_3\wedge w}{\det}.
\]
On the other hand, Equation \eqref{eq:mutaion formula for relative cycles} tells us that 
\[
A'_2=A_{\eta'_2}=A_{\eta'}A_{\eta_1-\eta_2}=\frac{v_0\wedge v_3\wedge w}{\det}\frac{\det}{\alpha_0\wedge v_2}=\frac{v_0\wedge v_3\wedge w}{\alpha_0\wedge v_2},
\]
which is precisely what we get in the cluster computation above.

%Figure \ref{fig:Example_m52_ClusterCoord}. These weaves represent an embedded exact Lagrangian surface $\Sigma(\ww)$ of genus one and one boundary component, i.e. a once-punctured Lagrangian torus bounding $m(5_2)$. Thus, we expect $b_1(\Sigma(\ww))=2$ vertices for the quiver, coming from a basis of $H_1(\Sigma(\ww),\Z)$. That said, the lollipops appearing in each of the two faces of $\bG$ (each of which giving a vertex) might, a priori, present an obstruction for the corresponding naive absolute cycles to be mutable, and thus each of this two vertices might or might not be mutable. We shall now explain that it is possible to find a basis for $H_1(\Sigma(\ww),\Z)$ where {\it one} of the cycles is mutable, but the other is not. The resulting quiver will hence be the $A_2$-quiver with one unfrozen vertex and one frozen vertex. This is explained as follows.


%\begin{center}
%	\begin{figure}[h!]
%		\centering
%		\includegraphics[width=\textwidth]{figures/Example_m52_ClusterCoord2.pdf}
%		\caption{.}
%		\label{fig:Example_m52_ClusterCoord2}
%	\end{figure}
%\end{center}


%	\begin{figure}[h!]
%		\centering
%		\includegraphics[width=\textwidth]{figures/Example_m52_ClusterCoord.pdf}
%		\caption{The weave discussed in Example \ref{ex:m52_ClusterCoord}, associated to one of the (two) maximal-tb Legendrian representatives of $m(5_2)$. The naive absolute and relative cycles are denoted by $\gamma_i$ and $\eta_i$ respectively, and $\gamma_1+\gamma_2,\gamma_2,\eta_1,\eta_2$ are drawn. The 3-dimensional decorated flags $F_i\in \GL(3,\C)/U$, satisfying the transversality conditions imposed by the weave, are points in the flag moduli $\fA(\ww)$.}
%		\label{fig:Example_m52_ClusterCoord}
%	\end{figure}

%The absolute cycles $\gamma_1,\gamma_2$ in Figure \ref{fig:Example_m52_Cycles} yield the cycles $\gamma_1+\gamma_2,\gamma_2$ in Figure \ref{fig:Example_m52_ClusterCoord}, which also depicts the corresponding naive relative cycles $\eta_1,\eta_2$. Note that neither of the naive absolute cycles, $\gamma_1$ nor $\gamma_2$ in Figure \ref{fig:Example_m52_Cycles}, are apparently mutable; again, this is the weave incarnation of the fact that the two faces of $\bG$ both contain a lollipop. (In particular, the naive dual cycles $\eta_1,\eta_2$ are thus not the initial relative cycles either.) Nevertheless, the cycle $\gamma_1+\gamma_2$, depicted in Figure \ref{fig:Example_m52_ClusterCoord}, is an $\sf I$-cycle and it is thus mutable. Therefore, we can consider $\gamma_1+\gamma_2$ as a mutable element of our basis for $H_1(\Sigma(\ww),\Z)$, and complete $\gamma_1+\gamma_2$ with either $\gamma_1$ or $\gamma_2$ to form a basis.\footnote{This ambiguity in this geometric choice gives rise to the quasi-cluster nature, in that we will be allowed to multiply by monomials in the frozens.} Let us choose $\{\gamma_1+\gamma_2,\gamma_2\}$ as our basis for $H_1(\Sigma(\ww),\Z)$, and then the dual relative basis is $\{\eta_1,\eta_2-\eta_1\}$. The $\SX$-quiver has $\gamma_1+\gamma_2$ as a mutable vertex, and $\gamma_2$ as a frozen vertex, with an arrow from the former to the latter. The $\SA$-quiver has $\eta_1$ as a mutable vertex, and $\eta_2-\eta_1$ as a frozen vertex, with an arrow from the former to the latter. Let us now discuss cluster variables associated to this quiver, for which we require the flag moduli for the weave $\ww$.

%The flag moduli $\fA(\ww)$ consists of tuples $(F_1,\ldots,F_{10})$ of 10 flags, up to $GL(3,\C)$ normalization, satisfying the transversality conditions imposed by the weave $\ww$. Here we denote each flag as a pair $F_i=(v_i,\alpha_i)$, where $v_i$ is a volume 1-form for the 1-dimensional subspace of $F_i$ and $alpha_i$ is a volume 2-form for the 2-dimensional subspace of $F_i$, both of which are embedded in $\C^3$. The transversality conditions of the weave impose the equations for $\fA(\ww)$. For instance, some transversality conditions which are readily read from Figure \ref{fig:Example_m52_ClusterCoord} are $$\alpha_1=\alpha_2,\quad v_1\wedge v_2=\alpha_2,\quad v_2=v_3,\quad \frac{\alpha_2\wedge\alpha_3}{v_2}=\mbox{det}_{\C^3},$$
%where again the last equation means we write $\alpha_2\wedge\alpha_3=\beta\wedge v_2$ and we impose $\beta=\det_{\C^3}$.

%\begin{center}
%	\begin{figure}[h!]
%		\centering
%		\includegraphics[width=\textwidth]{figures/Example_m52_ClusterCoord_Merodromies.pdf}
%		\caption{Slices of the weave $\ww$ in Example \ref{ex:m52_ClusterCoord} across the two naive relative cycles $\eta_1,\eta_2$. Note that the transversality conditions in $\fA(\ww)$ for the flags $F_i=(v_i,\alpha_i)$, $i\in[1,10]$, imply several equalities, such as $v_2=v_4$, $v_9=v_{10}$, $v_6=v_8$, $\alpha_2=\alpha_{10}$, $\a_4=\a_6$ and $\a_8=\a_9$.}
%		\label{fig:Example_m52_ClusterCoord_Merodromies}
%	\end{figure}
%\end{center}

%Let us now discuss the two microlocal merodromies $A_{\eta_1}$ and $A_{\eta_2-\eta_1}$ associated to the relative cycles $\eta_1$ and $\eta_2-\eta_1$. For that, we consider the braids $\beta(\eta_1)=\s_2\s_1\s_2$ and $\beta(\eta_2)=\s_1\s_2\s_1$, as drawn in Figure \ref{fig:Example_m52_ClusterCoord_Merodromies}, and insert the data of the corresponding flags $F_i$, also as depicted. Let us denote the standard volume form in $\C^3$ by $\det=\mbox{det}_{\C^3}$. Then, following Definition \ref{def:Avars}, we obtain
%$$A_{\eta_1}=\left(\frac{\a_4\stackrel{v_2}{\wedge}\a_2}{\det}\right)^0\cdot\left(\frac{v_2\wedge v_{10}}{\a_2}\right)^1\cdot\left(\frac{\a_2\stackrel{v_{10}}{\wedge}\a_9}{\det}\right)^1=\frac{v_2\wedge\a_9}{\det},$$
%$$A_{\eta_2}=\left(\frac{v_4\wedge v_{6}}{\a_4}\right)^0\cdot\left(\frac{\a_4\stackrel{v_{6}}{\wedge}\a_8}{\det}\right)^1\cdot \left(\frac{v_6\wedge v_{9}}{\a_8}\right)^1=\frac{\a_4\wedge v_9}{\det}.$$

%In consequence, since $\det$ is non-vanishing, both these functions $A_{\eta_1},A_{\eta_2}$ are global regular functions on the flag moduli $\fA(\ww)$. In order to understand the regularity and vanishing locus of the function $A_{\eta_2}A_{\eta_1}^{-1}$, the merodromy associated to the relative cycle $\eta_2-\eta_1$, we need to understand the flag moduli $\fA(\ww)$ better.

%First, we claim that $A_{\eta_2}A_{\eta_1}^{-1}$ is regular, i.e. that the vanishing of $A_{\eta_1}$ implies the vanishing of $A_{\eta_2}$. The vanishing of $A_{\eta_1}$, resp.~$A_{\eta_2}$, is the geometric condition that $v_2\in\a_9$, resp.~$v_9\in\a_4$. That is, we need to argue that a point $(F_1,\ldots,F_{10})$ with $F_2,F_9$ such that $v_2\in\a_9$ must also have that $v_9\in\a_4$. For that, note that $v_2\neq v_9$ in $\fA(\ww)$, $\a_4=\langle v_2,v_6\rangle$, since $v_4\neq v_6$ and $v_2=v_4$, and $a_9=\langle v_6,v_9\rangle$, as $v_8\neq v_9$ and $v_6=v_8$. Thus, it must be that $\a_4\cap \a_9=v_6$. The transversality conditions also state that $v_2\neq v_6$ and $v_6\neq v_9$. Hence, the condition $v_2\in\a_9$ implies $\a_{9}=\langle v_2,v_6\rangle=\a_{4}$, and hence $v_9\in\a_9=\a_4$ as required. This proves $A_{\eta_2}A_{\eta_1}^{-1}$ is a regular function.

%Second, we claim that $A_{\eta_2}A_{\eta_1}^{-1}$ is non-vanishing, which justifies $A_{\eta_2-\eta_1}$ being a frozen variable for $\fA(\ww)$. Indeed, by the same argument as above, the vanishing of $A_{\eta_2}$ implies the vanishing of $A_{\eta_1}$: the condition $v_9\in\a_4$ implies $\a_{4}=\langle v_6,v_9\rangle=\a_{9}$, and hence $v_2\in\a_4=\a_9$, as needed.



\subsection{Segon: an $m(7_2)$ Example}

We thank L.~Ng for asking a question, and participating in subsequent discussions, about the cluster structure on the moduli of sheaves singularly supported on a Legendrian representative of $m(7_2)$, which lead to the following example.

\begin{example}[The 4th Legendrian $m(7_2)$]\label{ex:4thm72} Let us consider the (-1)-closure of the 4-stranded positive braid word $$\beta=\sigma_1\sigma_3\sigma_3\sigma_3\sigma_2\sigma_2\sigma_3\sigma_1\sigma_2\sigma_2\sigma_3(\sigma_3\sigma_2\sigma_3\sigma_1\sigma_2\sigma_3)=\sigma_1\sigma_3\sigma_3\sigma_3\sigma_2\sigma_2\sigma_3\sigma_1\sigma_2\sigma_2\sigma_3\Delta,$$

\noindent This (-1)-closure describes a max-tb Legendrian representative $\La_4(m(7_2))\sse(\R^3,\xi_\st)$ in the smooth type $m(7_2)$, which in fact corresponds to the fourth entry in the part of the Legendrian Knot Atlas \cite{ChongchitmateNgPre} dedicate to $m(7_2)$. The second entry represents the Legendrian isotopy class of the (lift of the) alternating strand diagram of \ref{fig:Example_Twist} (upper right). The first and third entries do not admit binary Maslov indices, and thus do not arise as alternating strand diagrams of GP-graphs. We do not know whether this fourth Legendrian representative of $m(7_2)$ is the alternating strand diagram of a GP-graph; notice that it does admit a binary Maslov index, by virtue of being a (-1)-closure of a positive braid. Now, regardless of whether it arises from a GP-graph, the techniques and principles discovered in this article still apply, as follows.

\noindent Let us set $T$ to be a unique mark point, since $\La_4(m(7_2))$ is a knot. An embedded exact Lagrangian filling of $\La_4(m(7_2))$ is smoothly a once-punctured torus and since $H_1(L)=H_1(L,T)=\Z^2$, we can forgo keeping track of the unique marked point in $T$, which we do. Note that the Demazure product $$Dem(\sigma_1\sigma_3\sigma_3\sigma_3\sigma_2\sigma_2\sigma_3\sigma_1\sigma_2\sigma_2\sigma_3)=Dem(\sigma_1\sigma_3\sigma_2\sigma_3\sigma_1\sigma_2\sigma_3)=\sigma_1\sigma_3\sigma_2\sigma_3\sigma_1\sigma_2=w_0$$
is indeed $w_0$, and thus the Legendrian admits an embedded exact Lagrangian filling by \cite[Proposition 2.8]{CasalsNg}. In this case, there is no GP-graph $\bG$ from which we can build a weave $\ww(\bG)$ that represents a Lagrangian filling. Nevertheless, it is perfectly possible to do this by hand. In fact, there is an algorithmic procedure to produce weave fillings of (-1)-closures, using Demazure weaves, as explained in \cite[Section 4.7]{CGGS}. In either case, we have drawn a weave filling in Figure \ref{fig:Example_m72Alt}. Following the ideas and results from the manuscript, this dictates that the (mutation equivalence class of the) quiver ought to be the $A_2$-quiver, with $\gamma_1$ representing a mutable vertex and $\gamma_2$ representing a frozen vertex. The corresponding microlocal merodromies are associated to $\eta_1,\eta_2$, which we now compute in coordinates.

\begin{center}
	\begin{figure}[h!]
		\centering
		\includegraphics[scale=0.9]{figures/Example_m72Alt.pdf}
		\caption{A weave $\ww$ representating an embedded exact Lagrangian filling $L(\ww)$ of the Legendrian $\La_4(m(7_2))$, which is topologically a once-punctured torus. A basis of $H_1(L(\ww))=\Z^2$ is given by $\gamma_1,\gamma_2$, of which the 1-cycle $\gamma_1$ is $\L$-compressible. A dual basis of relative cycles for the dual lattice $H_1(L(\ww)\setminus T,\La_4(m(7_2))\setminus T)=\Z^2$ is given by the two relative 1-cycles $\eta_1,\eta_2$.}
		\label{fig:Example_m72Alt}
	\end{figure}
\end{center}

\noindent Let us introduce coordinates $z_1,\ldots,z_{17}\in\C$, corresponding to the crossings of $\beta$ left to right. Following the notation introduced in \cite[Section 5]{CasalsNg}, we can use the path matrix $P_\beta\in GL(4,\C)$ associated to the braid $\beta$ for $\La_4(m(7_2))$ in order to find implicit equations for the decorated moduli $\mathfrak{M}(\La_4(m(7_2)),T)$, as it coincides with the augmentation variety. Explicitly, by \cite[Proposition 5.2]{CasalsNg}, this moduli is cut out by the entry-wise equations $P_\beta+\mbox{Id}_4=0$. The microlocal monodromies associated to $\eta_1$ and $\eta_2$ are
$$A_{\eta_1}=z_2,\quad A_{\eta_2}=-z_5,$$
both of them being understood as the restrictions of the ambient functions $z_2,z_5\in\C[z_1,\ldots,z_{17}]$ to $\mathfrak{M}(\La_4(m(7_2)),T)\sse\C^{17}$. Still in the notation of \cite{CasalsNg}, we set $t_1=t_2=t_3=1$ and $t_4=-1$ with regards to the marked point in $T$. Note that the general theory states that $A_{\eta_2}$ is a frozen variable, and thus our first computation in this explicit example should verify that the ambient regular function $z_5$ is non-vanishing on the affine subvariety $\mathfrak{M}(\La_4(m(7_2)),T)$. Indeed, consider the set $\mathbb{P}$ of the 16 polynomial entries of $P_\beta+\mbox{Id}_4$. Then a Gr\"obner basis for $\C[z_1,\ldots,z_{17}]/\langle\mathbb{P},z_5\rangle$, whose spectrum is the intersection $\mathfrak{M}(\La_4(m(7_2)),T)\cap\{z_5=0\}$, can be computed to be $\{1\}$, e.g.~using Mathematica. In consequence, the intersection is empty and the function $z_5$ does not vanish on $\mathfrak{M}(\La_4(m(7_2)),T)$. The second computation is that $A_{\eta_1}$, the only mutable variable, does indeed mutate to a regular function. Given the quiver, the mutated variable is
$$A'_{\eta_1}=\frac{1+A_{\eta_2}}{A_{\eta_1}}=\frac{1-z_5}{z_2}.$$
Now, $A_{\eta_1}=z_2$ certainly vanishes on $\mathfrak{M}(\La_4(m(7_2)),T)$, but we can verify that, when restricted to $\mathfrak{M}(\La_4(m(7_2)),T)$, if $z_2$ vanishes, then so does $1-z_5$. Indeed, a Gr\"obner basis for the subvariety
$$\mathfrak{M}(\La_4(m(7_2)),T)\cap\{z_2=0\}\sse\C^{17}$$
is computed to be
\small
$$\left\{z_{16}-1,z_{15}-1,z_{14}-1,z_{13},z_{12}+1,z_{11}-1,z_{10}-1,z_9+1,z_8,z_7,z_6+1,\color{blue}z_5-1\color{black},z_4,z_3-z_{17},z_1-1\right\}.$$
\normalsize
This Gr\"obner basis contains the element $z_5-1$, highlighted in blue above, and we conclude that $A'_{\eta_1}$ is a regular function on $\mathfrak{M}(\La_4(m(7_2)),T)$, as desired.

\noindent As a last verification, let us explicitly compute that the intersection
$$T_{z_2,z_5}:=\mathfrak{M}(\La_4(m(7_2)),T)\cap\{z_2\neq0,z_5\neq0\}\sse\C^{17}$$
is indeed an algebraic torus $(\C^*)^2$ whose coordinate ring can be identified with the Laurent polynomial ring $\C[z_2^{\pm1},z_5^{\pm1}]$. A Gr\"obner basis for the coordinate ring of this intersection $T_{z_2,z_5}$ is
$$\left\{\frac{z_{16}}{z_2}+z_{17}-\frac{1}{z_2},z_{15}-1,z_{14}-1,z_{13},z_{17} z_{12}-\frac{z_{12}}{z_2}-\frac{1}{z_2},z_{12} z_{16}+1,z_{11}-z_{16},\right.$$
$$z_{10}-z_{16},z_9-z_{12},z_8,z_7,z_6-z_{12},z_5-z_{16},\frac{z_4}{z_2}+z_{16},-z_{16}^2+z_{16}+z_4 z_{17},$$
$$\left.z_3+\frac{z_{12}}{z_2}+\frac{1}{z_2},z_2-z_4 z_{12},z_1-z_{16}\right\},$$
which readily tells us that $z_7=z_8=z_{13}=0$ and $z_{14}=z_{15}=1$ when we restrict to $T_{z_2,z_5}$. Also, we learn that
$$z_1=-z_6^{-1}=-z_9^{-1}=z_{10}=z_{11}=-z_{12}^{-1}=z_{16}=z_{5}$$
and thus all these coordinates are graphs on the coordinate $z_5$. The remaining variables are $z_2,z_3,z_4$. Since the element $z_4z_2^{-1}+z_{16}$ is in the basis, or equivalently $z_2-z_4z_{12}$, we have that $z_4=-z_2z_5$, and thus $z_4$ is graphical on the pair $z_2,z_5$. The presence of $z_3+z_{12}z_2^{-1}+z_2^{-1}$ in the basis implies that $z_3=-z_2^{-1}(1-z_5^{-1})$. This concludes that $z_1,z_3,z_4,z_6,z_7,\ldots,z_{17}$ are graphical on $z_2^{\pm1},z_5^{\pm1}$ in the above intersection $T_{z_2,z_5}$, and that $z_2,z_5$ have no relations among them: $T_{z_2,z_5}$ is algebraically isomorphic to $\C[A_{\eta_1}^{\pm1},A_{\eta_2}^{\pm1}]\cong \C[z_2^{\pm1},z_5^{\pm1}]\cong(\C^*)^2$ as desired. A similar computation shows that $\C[(A'_{\eta_1})^{\pm1},A_{\eta_2}^{\pm1}]$ is an algebraic torus $(\C^*)^2$ as well.
\hfill$\Box$
\end{example}

